POD-based reduced order methods for optimal control problems governed by parametric partial differential equation with varying boundary control

In this work we propose tailored model order reduction for varying boundary optimal control problems governed by parametric partial differential equations. With varying boundary control, we mean that a specific parameter changes where the boundary control acts on the system. This peculiar formulation might benefit from model order reduction. Indeed, fast and reliable simulations of this model can be of utmost usefulness in many applied fields, such as geophysics and energy engineering. However, varying boundary control features very complicated and diversified parametric behaviour for the state and adjoint variables. The state solution, for example, changing the boundary control parameter, might feature transport phenomena. Moreover, the problem loses its affine structure. It is well known that classical model order reduction techniques fail in this setting, both in accuracy and in efficiency. Thus, we propose reduced approaches inspired by the ones used when dealing with wave-like phenomena. Indeed, we compare standard proper orthogonal decomposition with two tailored strategies: geometric recasting and local proper orthogonal decomposition. Geometric recasting solves the optimization system in a reference domain simplifying the problem at hand avoiding hyper-reduction, while local proper orthogonal decomposition builds local bases to increase the accuracy of the reduced solution in very general settings (where geometric recasting is unfeasible). We compare the various approaches on two different numerical experiments based on geometries of increasing complexity.

==> Sections/App_forms.tex <==
\section{Geo-R computations for Section \ref{sec:results}}
\label{A:2}

==> Sections/App_th.tex <==
\section{Direct computation of $\overline{\beta_{LB}}(\bmu)$}
\label{A:1}
In this Appendix, we provide the proof of Theorem \ref{Th:1}. For the sake of clarity we recall it below.
\begin{theorem*}
    Given the bilinear form $\mathcal B : Y \times Y \to \mathbb{R}$ as in \eqref{eq:B} and the Babu\v ska  inf-sup stability constant $\beta_h(\bmu)$ as in \eqref{infsup_hf}
    and taken the lower bound $\overline{\beta_{LB}}(\bmu)$ defined in \eqref{eq:over}
%    where $\gamma_a(\bmu)$, $\gamma_T(\bmu)$ and $c_{\Omega}$ are the constant s.t. for all $y \in Y$:
%    \begin{equation*}
%        a(y, y) \geq \gamma_a(\bmu) \norm{y}^2_Y, \quad
%        \norm{y}_{U} \leq\gamma_T(\bmu)\norm{y}_Y \quad \text{and} \quad
%        \norm{y}_{L^2(\Omega)} \leq c_{\Omega}\norm{y}_Y.
%    \end{equation*}
%    $\Rightarrow$
then
    % \begin{equation*}
        $\beta_h(\bmu) \geq \overline{\beta_{LB}}(\bmu).$
    % \end{equation*}
\end{theorem*}

\begin{proof}
    Starting from the definition of $\beta_h(\bmu)$ we choose $\tilde{w}\disc := y\disc + c_1 p\disc$ and $\tilde{q}\disc := c_2 y\disc - p\disc$ and we obtain:
    \begin{equation*}
        \beta_h(\bmu) \geq  \inf_{(y\disc, p\disc)} \frac{\Cal B((y\disc, p\disc), (\tilde{w}\disc, \tilde{q}\disc); \bmu)}{\sqrt{\norm{y\disc}_{Y}^2 + \norm{p\disc}_{Y}^2} \sqrt{\norm{\tilde{w}\disc}_{Y}^2 + \norm{\tilde{q}\disc}_{Y}^2}}.
    \end{equation*}
    We separately analyze the numerator $\mathsf n$ and the denominator $\mathsf d$ of \eqref{eq:B} omitting the superscript symbol $\disc$.
    Substituting the definitions $\tilde{w}$ and $\tilde{q}$ in the numerator we obtain:
    \begin{eqnarray*}
        \mathsf n & \eqdot &m(y, y + c_1 p; \bmu) + a(y + c_1 p, p; \bmu) + a(y, c_2 y - p; \bmu) - \frac{1}{\alpha} c(p, c_2 y - p; \bmu) =\\
        &&c_2 a(y, y; \bmu) + c_1 a(p, p; \bmu) + \frac{1}{\alpha} c(p, p; \bmu) - \frac{c_2}{\alpha} c(p, y; \bmu) + m(y, y; \bmu) + c_1 m(y, p; \bmu)
    \end{eqnarray*}
    Now, recalling that $\gamma_a(\bmu)$ is the coercity constant of the bilinear form $a(\cdot, \cdot;\bmu)$
%    \begin{equation*}
%        a(y, y) \geq \gamma_a(\bmu) \norm{y}^2_Y,
%    \end{equation*}
    we obtain:
    \begin{equation*}
        \mathsf n \geq c_2 \gamma_a(\bmu) \norm{y}^2_Y + c_1 \gamma_a(\bmu) \norm{p}^2_Y + \frac{1}{\alpha} c(p, p) - \frac{c_2}{\alpha} c(p, y) + m(y, y) + c_1 m(y, p).
    \end{equation*}
    Now, given $\epsilon > 0$, we employ the Young's inequality starting from 
$$(a\pm\epsilon b) ^ 2 \geq 0 \quad \Rightarrow \quad \pm ab \geq -\frac{a^2}{2 \epsilon} - \frac{\epsilon b^2}{2};$$
we applied it on the bilinear forms 
$$c(y, p) = \int_{\Gamma_{C}^{\mu_u}}y p \quad \text{ and } \quad m(y, p) = \int_{\Omega_{\text{obs}}} yp,$$ respectively, with constants $\varepsilon, \eta > 0$, obtaining:
    \begin{eqnarray*}
        \mathsf n & \geq & c_2 \gamma_a(\bmu) \norm{y}^2_Y + c_1 \gamma_a(\bmu) \norm{p}^2_Y + \frac{1}{\alpha} \norm{p}^2_U - \frac{c_2}{2 \alpha \varepsilon} \norm{p}^2_{U} - \frac{c_2 \varepsilon}{2 \alpha} \norm{y}^2_{U}\\
        &&\qquad \qquad \qquad \qquad \qquad \qquad
+\norm{y}^2_{L^2(\Omega_{\text{obs}})} - \frac{c_1 \eta}{2} \norm{y}^2_{L^2(\Omega_{\text{obs}})} - \frac{c_1}{2 \eta} \norm{p}^2_{L^2(\Omega_{\text{obs}})}.
    \end{eqnarray*}
We recall the role of $\gamma_T(\bmu)$ and $C_{\Omega}$ as the trace and the Poincar\'e constants
% s.t. for all $y \in Y$:
%    \begin{equation*}
%        \norm{y}_{U} \leq\gamma_T(\bmu)\norm{y}_Y \quad \text{and} \quad
%        \norm{y}_{L^2(\Omega)} \leq c_{\Omega}\norm{y}_Y,
%    \end{equation*}
    and we obtain:
    \begin{eqnarray}
        \label{eq:N_lastStep}
        \quad \quad \quad  \mathsf n & \geq & \frac{c_2}{2} \gamma_a (\bmu)\norm{y}^2_Y + \frac{c_2}{2} \left (\gamma_a(\bmu) - \frac{\varepsilon \gamma_T(\bmu)}{\alpha}\right ) \norm{y}^2_Y + \frac{c_1}{2} \gamma_a(\bmu) \norm{p}^2_Y \\
        && \qquad \qquad 
+ \frac{c_1}{2} \left (\gamma_a(\bmu)  - \frac{c_{\Omega}}{\eta} \right ) \norm{p}^2_Y  + \frac{1}{\alpha}\left (1 - \frac{c_2}{2 \varepsilon} \right ) \norm{p}^2_U + \left (1 - \frac{c_1 \eta}{2} \right ) \norm{y}^2_{L^2(\Omega_{\text{obs}})}.\nonumber
    \end{eqnarray}
    Now we explicit all the constants to be determined imposing:
    \begin{equation*}
        \left (\gamma_a (\bmu) - \frac{\varepsilon \gamma_T(\bmu)}{\alpha}\right ) = 0, \quad \left (\gamma_a(\bmu)  - \frac{c_{\Omega}}{\eta}\right ) = 0, \quad \left (1 - \frac{c_2}{2 \varepsilon}\right ) = 0, \quad \left (1 - \frac{c_1 \eta}{2} \right ) = 0,
    \end{equation*}
    and we obtain:
    \begin{equation}
        \label{eq:constants}
        \varepsilon = \frac{\alpha \gamma_a(\bmu)}{\gamma_T(\bmu)}, \quad \eta = \frac{C_{\Omega}}{\gamma_a(\bmu)}, \quad c_2 = \frac{2 \alpha \gamma_a(\bmu)}{\gamma_T(\bmu)}, \quad c_1 = \frac{2 \gamma_a(\bmu)}{c_{\Omega}}.
    \end{equation}
    Finally, we substitute the constants obtained in \eqref{eq:N_lastStep}, we have:
    \begin{equation}
        \label{eq:numerator}
        \mathsf n  \geq \frac{\alpha \gamma_a^2(\bmu)}{\gamma_T(\bmu)} \norm{y}^2_Y + \frac{\gamma_a^2(\bmu)}{C_{\Omega}} \norm{p}^2_Y \geq \gamma_a^2(\bmu) \min \left \{ \frac{\alpha}{\gamma_T(\bmu)}, \frac{1}{C_{\Omega}}\right \} (\norm{y}^2_Y + \norm{p}^2_Y).
    \end{equation}
    We now focus on the denominator 
    \begin{equation*}
        \mathsf d \eqdot \sqrt{\norm{y}_{Y}^2 + \norm{p}_{Y}^2} \sqrt{\norm{ y + c_1 p}_{Y}^2 + \norm{c_2 y - p}_{Y}^2}.
    \end{equation*}
    We use the Pythagorean theorem on $\norm{\cdot}^2_Y$ and again the Young's inequality obtaining:
    \begin{eqnarray*}
        \mathsf d &\leq& \sqrt{\norm{y}_{Y}^2 + \norm{p}_{Y}^2} \sqrt{\norm{y}_Y^2 + c_1^2 \norm{p}_{Y}^2 + 2 c_2^2 \norm{y}_Y^2 + 2 \norm{p}_{Y}^2} \\
        & \leq&  \max\left \{\sqrt{2c_2^2+1}, \sqrt{c_1^2 + 2} \right \}(\norm{y}_{Y}^2 + \norm{p}_{Y}^2)
    \end{eqnarray*}
    Finally, using the constants of equation \eqref{eq:constants} we have:
    \begin{equation}
        \label{eq:denominator}
        \mathsf d \leq \max \left \{\sqrt{\frac{8\alpha^2\gamma_a^2(\bmu)}{\gamma_T^2(\bmu)}+1}, \sqrt{\frac{4 \gamma_a^2(\bmu)}{C_{\Omega}^2} + 2} \right \}(\norm{y}_{Y}^2 + \norm{p}_{Y}^2)
    \end{equation}
    The proof ends collecting together the estimation of equations \eqref{eq:numerator} and \eqref{eq:denominator}, since the state and the adjoint variables are arbitrary.
\end{proof}
